Multi-microphone Automatic Speech Segmentation in Meetings Based on Circular Harmonics Features

Speaker diarization is the task of answering Who spoke and when? in an audio stream. Pipeline systems rely on speech segmentation to extract speakers' segments and achieve robust speaker diarization. This paper proposes a common framework to solve three segmentation tasks in the distant speech scenario: Voice Activity Detection (VAD), Overlapped Speech Detection (OSD), and Speaker Change Detection (SCD). In the literature, a few studies investigate the multi-microphone distant speech scenario. In this work, we propose a new set of spatial features based on direction-of-arrival estimations in the circular harmonic domain (CH-DOA). These spatial features are extracted from multi-microphone audio data and combined with standard acoustic features. Experiments on the AMI meeting corpus show that CH-DOA can improve the segmentation while being robust in the case of deactivated microphones.

==> 01_intro.tex <==
\section{Introduction}

Speaker diarization is the task of answering \textit{Who spoke and when?} in an audio stream~\cite{anguera2012speaker,park2022review}.
Many speaker diarization approaches are based on pipeline architectures~\cite{park2022review,bredin_pyannoteaudio_2020,landini2022bayesian}.
Those approaches rely on a speech segmentation step that extracts speaker-homogeneous segments. %estimates speech segments containing one active speaker. 
Speaker clustering is then performed by extracting and grouping speaker embeddings via clustering algorithms~\cite{park2022review}.
This paper focuses on automatic speech segmentation, which can be divided into three sub-tasks: Voice Activity Detection (VAD), Overlapped Speech Detection (OSD), and Speaker Change Detection (SCD).

VAD detects speech segments in the audio signal. %from non-speech ones in the audio signal. 
It is the first step in most speaker diarization pipelines~\cite{park2022review}.
%SCD is required to detect speaker turns in the audio signal, i.e., when the currently active speaker is changing.
%Finally, overlapping speech is one of the major sources of errors in speaker diarization pipelines~\cite{bredin21_interspeech,garcia2019speaker}.
%OSD consists in detecting speech segments in which multiple speakers are simultaneously active and is required for robust diarization.
%Early studies on VAD~\cite{sohn1999statistical,ng2012developing}, OSD~\cite{boakye_improved_2011,charlet_impact_2013,yella2014overlapping} and SCD~\cite{siegler1997automatic,liu1999fast} are based on the statistical modeling of acoustic features with HMM/GMM approaches. 
%The latter is originally solved by comparing the statistics of two adjacent segments using HMM/GMM models.
Although early studies on VAD are mostly based on signal processing and statistical modeling~\cite{sohn1999statistical,ng2012developing}, current approaches exploit the strong modeling capacities of deep neural networks~\cite{ryant2013speech,bredin21_interspeech,Cornell2022,lavechin2019end}.
Specifically, Lavechin~\textit{et al.}~\cite{lavechin2019end} show that VAD can be solved as a binary frame classification task.

OSD consists in detecting speech segments in which multiple speakers are simultaneously active.
Overlapping speech is one of the major sources of errors in speaker diarization pipelines~\cite{bredin21_interspeech,garcia2019speaker}.
Similarly to VAD, early OSD studies are based on HMM/GMM models~\cite{boakye2008overlapped,charlet_impact_2013,yella2014overlapping}.
Current approaches exploit neural networks to classify acoustic features at the frame level~\cite{bredin21_interspeech,Cornell2022,lebourdais22_interspeech}.

SCD consists in detecting speaker turns in the audio signal, i.e., when the currently active speaker is changing.
Early studies detect turns by comparing the statistics of two successive speech segments~\cite{siegler1997automatic,liu1999fast}.
Current approaches exploit neural networks.
In~\cite{yin2017speaker}, authors show that SCD can be solved similarly to VAD or OSD as a binary frame classification task.
This task is solved as a regression task in~\cite{hruz2017convolutional} by predicting functions in which maxima are located at turn locations.

Most VAD, OSD, and SCD studies are conducted on single-channel data. 
In the meeting context, recording signals with a distant device offers practical benefits since it does not require participants to carry an individual microphone.
Microphone arrays are commonly used as distant devices to capture additional spatial information.
Few studies have been conducted on multi-microphone speech segmentation~\cite{Cornell2022,hu2015speaker,cornell_detecting_2020,mariotte22_interspeech}.
In particular, Cornell~\textit{et al.}~\cite{Cornell2022} explore the use of Interaural Phase Difference (IPD) spatial features for joint VAD and OSD and reported a noticeable performance gain.
Hu~\textit{et al.}~\cite{hu2015speaker} investigate the use of Time Difference of Arrival (TDOA) features to detect speaker changes. 
Although the authors show diarization performance gain, experiments were conducted on simulated data.
To the best of our knowledge, no other work has been reported on the use of spatial features for distant SCD. 
Although several spatial features have been investigated in various multi-microphone speech processing tasks~\cite{pak2019sound,vincent2018audio,gu2020enhancing}.
In particular, SongGong~\textit{et al.}~\cite{songgong_robust_2021} propose a speaker localization method based on circular harmonics (CH).
Although these features require the use of a circular array, they depend little on the number of available microphones.
Hence, circular harmonics are an interesting framework for feature extraction to rely less on the array configuration.

In this paper, we tackle VAD, OSD, and SCD tasks with the same architecture. 
We propose the use of CH to extract spatial features for multi-microphone speech segmentation.
This choice is motivated by the common use of circular microphone arrays to capture distant speech in meetings~\cite{carletta2006ami,fu21b_interspeech}.
The proposed spatial features consist of direction of arrival (DOA) estimation in the CH framework.
Spatial features are combined with commonly used acoustic features to solve VAD, OSD, and SCD.
%To the best of our knowledge, 
As far as authors are aware, this is the first investigation on the use of CH features for distant speech segmentation.
Furthermore, we report the impact of IPD spatial features for SCD since no work has been found considering their use for this task.
We demonstrate that adding spatial information drastically improves the detection of speaker turns.
Finally, we present encouraging results of CH-DOA-based OSD and SCD systems under mismatched array conditions.
The code will be available soon in a large-scale diarization toolkit\footnote{Hidden for anonymization purpose.}.
%The code will be available soon in a large-scale diarization toolkit\footnote{\url{https://git-lium.univ-lemans.fr/speaker}}.
%Finally, the impact of spatial features is evaluated in a full speaker diarization pipeline.

The paper is organized as follows. Sect.~\ref{sect:tasksssssssssssssss} presents VAD, OSD, and SCD tasks. Sect.~\ref{sect2_ch_feat} presents the CH-DOA feature extraction.
Sect.~\ref{sect3_protocol} introduces the speech segmentation model along with the dataset and the experimental protocol before presenting results in Sect.~\ref{sect4_seg_perf} and conclusions in Section~\ref{sect_ccl}.



==> 05_vbx.tex <==
\section{Impact on speaker diarization}

This section evaluates the impact of the proposed CH features on the diarization performance.

\subsection{Speaker Diarization system}



\subsection{Results}

\begin{table}[ht!]
    \centering
    \caption{Diarization performance with several VAD segmentations.}
    \begin{tabular}{lccc}
    \toprule
         DER$_{\%\downarrow}$     & Forgiving & Fair & Full\\ \midrule
         Log-Mel & \textbf{9.7} & 18.6 & \textbf{26.8} \\
         \quad + CSIPD & 10.5 & \textbf{16.7} & 28.2\\
         \quad + DOAS & \textbf{9.6} & 18.8 & \textbf{27.3}\\
         \bottomrule
    \end{tabular}
    \label{tab:der_res}
\end{table}
